A 2-approximation for the $k$-prize-collecting Steiner tree problem

We consider the $k$-prize-collecting Steiner tree problem. An instance is composed of an integer $k$ and a graph $G$ with costs on edges and penalties on vertices. The objective is to find a tree spanning at least $k$ vertices which minimizes the cost of the edges in the tree plus the penalties of vertices not in the tree. This is one of the most fundamental network design problems and is a common generalization of the prize-collecting Steiner tree and the $k$-minimum spanning tree problems. Our main result is a 2-approximation algorithm, which improves on the currently best known approximation factor of 3.96 and has a faster running time. The algorithm builds on a modification of the primal-dual framework of Goemans and Williamson, and reveals interesting properties that can be applied to other similar problems.

==> pseudocode/pv_latin.tex <==

\begin{algorithm}[htb!]
	\DontPrintSemicolon
	\caption{$\PV(\pot,\tblist)$}
	\label{subsec:PV:alg:PV}

	\uIf{\textnormal{$\GW(\pot,\tblist)$ returns at least $k$ vertices}} {
		Let $(\tblist_\subplus, \tblist_\subminus) \gets (\tblist, \sublist)$
	}
	\Else{
		Let $(\tblist_\subplus, \tblist_\subminus) \gets (\sublist, \tblist)$
	}

	Let $(T_\subminus,\calb_\subminus) \gets \GP(\pot,\tblist_\subminus)$
	and $\call_\subminus$ be the computed laminar collection\;

	Let $(T_\subplus,\calb_\subplus) \gets \GP(\pot,\tblist_\subplus)$\;

	Let $H \gets T_\subminus \cup T_\subplus$ and $\hath \gets \PP(H,\calb_\subplus)$\;

	\nonl\;

	\tcp*[h]{finding a subset path}\;
	\uIf{\textnormal{$\tblist_{|\tblist|}$ is a subset}}{
		Obtain sequence $D_1,D_2,\dots,D_\ell$ as described in the algorithm
	}
	\Else
	{
		Obtain sequence $D_1,D_2,\dots,D_\ell$ as described in the algorithm
	}
	Find largest $t$ such that $D_t,D_{t+1}, \dots,D_{\ell+1}$ cover at least $k$ vertices

	\nonl\;
	\tcp*[h]{picking-vertices}\;
	Let $P_0 \gets D_{t+1}$, $i \gets 1$ and $m \gets k - \sum_{i=t+1}^{\ell+1} |D_i|$\;
	Find a neighbor $v$ of $P_0$ in $D_t$\;
	Find $B_t \in \calb_\subminus$ such that $D_t \subseteq B_t$ and let $S \gets B_t$\;
	\While{\textnormal{$m \ne 0$}}
	{
		\uIf{\textnormal{$m = 1$}}
		{
			Define $P_i \gets \{v\}$ and $s \gets i$\;
			Let $m \gets 0$ and stop the loop\;
		}
		\Else{
			Find $S_1, S_2 \in \call_\subminus$ with $S = S_1 \cup S_2$ and $v \in S_1$\;
			\uIf{\textnormal{$|S_1 \cap D_t| \ge m$}}
			{
				Let $S \gets S_1$\;
			}\Else{
				Find an edge with extremes $v_1 \in S_1$ and $v_2 \in S_2$\;
				Let $P_i \gets S_1 \cap D_t$, $m \gets m - |P_i|$\;
				Let $S \gets S_2$ and $v \gets v_2$.\;
				Let $i \gets i + 1$\;
			}
		}
	}
	\nonl\;
	Let $T$ be the tree induced by sequence $P_s, \dots, P_1, D_{t+1}, \dots, D_{\ell+1}$\;
	\Return{T}
\end{algorithm}

